An Optimal and Model-Independent Measurement of the Intracluster Pressure Profile I: Methodology and First Applications

We present a statistically-optimal and model-independent method to extract the pressure profile of hot gas in the intracluster medium (ICM). Using the thermal Sunyaev-Zeldovich effect, we constrain the mean pressure profile of the ICM by appropriately considering all primary cosmic microwave background (CMB) and instrumental noise correlations, while using the maximum resolution and sensitivity of all frequency channels. As a first application, we analyze CMB maps of WMAP 9-year data through a study of the Meta-Catalogue of X-ray detected Clusters of galaxies (MCXC). We constrain the universal pressure profile out to 4R_500 with 15-sigma confidence, though our measurements are only significant out to R_200. Using a temperature profile constrained from X-ray observations, we measure the mean gas mass fraction out to R_200. Within statistical and systematic uncertainties, our constraints are compatible with the cosmic baryon fraction and the expected gas fraction in halos. While Planck multi-frequency CMB data are expected to reduce statistical uncertainties by a factor of 20, we argue that systematic errors in determining mass of clusters dominate the uncertainty in gas mass fraction measurements at the level of 20 percent.

==> normedCM_162.tex <==
 &  Bin 1 & Bin 2 & Bin 3 & Bin 4 & Bin 5 & Bin 6 & Bin 7 & Bin 8 \\
\hline
 Bin 1 &  1.000 & -0.612 & 0.277 & -0.069 & 0.033 & -0.024 & -0.001 & -0.011 \\
 Bin 2 &  -0.612 & 1.000 & -0.497 & 0.232 & -0.039 & -0.007 & -0.023 & -0.043 \\
 Bin 3 &  0.277 & -0.497 & 1.000 & -0.445 & 0.147 & -0.013 & -0.041 & -0.044 \\
 Bin 4 &  -0.069 & 0.232 & -0.445 & 1.000 & -0.434 & 0.091 & -0.015 & -0.075 \\
 Bin 5 &  0.033 & -0.039 & 0.147 & -0.434 & 1.000 & -0.451 & 0.108 & -0.053 \\
 Bin 6 &  -0.024 & -0.007 & -0.013 & 0.091 & -0.451 & 1.000 & -0.442 & 0.085 \\
 Bin 7 &  -0.001 & -0.023 & -0.041 & -0.015 & 0.108 & -0.442 & 1.000 & -0.476 \\
 Bin 8 &  -0.011 & -0.043 & -0.044 & -0.075 & -0.053 & 0.085 & -0.476 & 1.000 \\


==> normedCM_all.tex <==
 &  Bin 1 & Bin 2 & Bin 3 & Bin 4 & Bin 5 & Bin 6 & Bin 7 & Bin 8 \\
\hline
 Bin 1 &  1.000 & -0.727 & 0.282 & -0.082 & 0.029 & -0.022 & 0.011 & -0.001 \\
 Bin 2 &  -0.727 & 1.000 & -0.671 & 0.214 & -0.051 & 0.005 & -0.003 & 0.006 \\
 Bin 3 &  0.282 & -0.671 & 1.000 & -0.633 & 0.144 & 0.000 & -0.023 & 0.018 \\
 Bin 4 &  -0.082 & 0.214 & -0.633 & 1.000 & -0.598 & 0.109 & 0.009 & -0.014 \\
 Bin 5 &  0.029 & -0.051 & 0.144 & -0.598 & 1.000 & -0.594 & 0.117 & -0.004 \\
 Bin 6 &  -0.022 & 0.005 & 0.000 & 0.109 & -0.594 & 1.000 & -0.597 & 0.156 \\
 Bin 7 &  0.011 & -0.003 & -0.023 & 0.009 & 0.117 & -0.597 & 1.000 & -0.697 \\
 Bin 8 &  -0.001 & 0.006 & 0.018 & -0.014 & -0.004 & 0.156 & -0.697 & 1.000 \\

